A dynamical model of supernova feedback: gas outflows from the interstellar medium

We present a dynamical model of supernova feedback which follows the evolution of pressurised bubbles driven by supernovae in a multi-phase interstellar medium (ISM). The bubbles are followed until the point of break-out into the halo, starting from an initial adiabatic phase to a radiative phase. We show that a key property which sets the fate of bubbles in the ISM is the gas surface density, through the work done by the expansion of bubbles and its role in setting the gas scaleheight. The multi-phase description of the ISM is essential, and neglecting it leads to order of magnitude differences in the predicted outflow rates. We compare our predicted mass loading and outflow velocities to observations of local and high-redshift galaxies and find good agreement over a wide range of stellar masses and velocities. With the aim of analysing the dependence of the mass loading of the outflow, beta (i.e. the ratio between the outflow and star formation rates), on galaxy properties, we embed our model in the galaxy formation simulation, GALFORM, set in the LCDM framework. We find that a dependence of beta solely on the circular velocity, as is widely assumed in the literature, is actually a poor description of the outflow rate, as large variations with redshift and galaxy properties are obtained. Moreover, we find that below a circular velocity of 80km/s the mass loading saturates. A more fundamental relation is that between beta and the gas scaleheight of the disk, hg, and the gas fraction, fgas, as beta hg^(1.1) fgas^(0.4), or the gas surface density, \Sigma_g, and the gas fraction, as beta \Sigma_g^(-0.6) fgas^(0.8). We find that using the new mass loading model leads to a shallower faint-end slope in the predicted optical and near-IR galaxy luminosity functions.

==> Makefile <==
SHELL=/bin/bash
NOMBRE=$(shell grep -H \\documentclass *.tex | cut -d: -f1 | cut -d. -f1)

ifeq ($(strip $(wildcard $(NOMBRE).bib) ),)
HAVE_BIB=no
else
HAVE_BIB=yes
endif



DEPENDENCIES=$(NOMBRE).tex

ifeq '$(HAVE_BIB)' 'yes'
DEPENDENCIES+= $(NOMBRE).bib
endif

HAVE_BIB=yes

all: $(NOMBRE).pdf

$(NOMBRE).pdf: $(DEPENDENCIES)
	@echo "   Making dvi for first time..."
	@latex -halt-on-error $(NOMBRE).tex &> .my_log || (cat .my_log && rm .my_log && exit 1)
	@rm .my_log
	@if [[ "${HAVE_BIB}" == "yes" ]]; then \
	echo "   Compiling references..." && \
	(bibtex $(NOMBRE) &> .my_log || (cat .my_log && rm .my_log && exit 1)) && \
	rm .my_log && \
	echo "   Re-making dvi including bibliography..." && \
	latex $(NOMBRE).tex &> /dev/null; \
	fi
	@echo "   Re-making dvi for satisfying references..."
	@latex $(NOMBRE).tex &> /dev/null
	@echo "   Generating final pdf..."
	@dvipdf $(NOMBRE).dvi &> /dev/null

clean:
	-rm -f $(NOMBRE).{aux,toc,log,tmp,dvi,idx,ilg,ind,bbl,blg,out} .my_log

distclean: clean
	-rm -f $(NOMBRE).pdf

k: $(NOMBRE).pdf
	@echo "   Opening $(NOMBRE).pdf with evince..."
	@evince $(NOMBRE).pdf &> /dev/null &

x: $(NOMBRE).pdf
	@echo "   Opening $(NOMBRE).pdf with xpdf..."
	@xpdf $(NOMBRE).pdf &> /dev/null &


==> app_numerical_tests.tex <==
\section[]{Numerical integration of the motion and mass conservation equations of bubbles}\label{App:NumSols}

To solve for the evolution of individual bubbles we use an hybrid method 
invoking analytic solutions for the initial adiabatic phase and a numerical solution of the radiative phase. 
We apply the set of analytical solutions for the first $2/3$ of cooling time, $t=2/3\,t_{\rm cool}$, and 
track the posterior evolution with the numerical technique of Runge-Kutta with adaptive stepsizes \citep{NR}.
The accuracy we use to solve the differential equations is a non-critical factor as we show in 
Fig.~\ref{ConvTest2c}. Properties of bubbles are usually quickly converged (after few timesteps), even for the best 
accuracies.

\begin{figure}
\begin{center}
\includegraphics[width=0.47\textwidth]{Figs/BubblesTesting_1c_Bow06.BR.SNdyn.eps}
\caption{Convergence test for the accuracy to which differential 
equations for the evolution of bubbles are solved. Momentum, radius, velocity, bubble or shell mass (depending on the evolutionary stage),
internal metallicity and internal mass of bubbles
as a function of time when varying the accuracy as labelled.}
\label{ConvTest2c}
\end{center}
\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[width=0.47\textwidth]{Figs/BubblesTesting_InitialCond_Bow06.BR.SNdyn.eps}
%\caption{Convergence test for the initial conditions of the SNe dynamical model. 
%Thermal energy, radius, velocity, bubble or shell mass (depending on the evolutionary stage), 
%internal metallicity and internal mass ($>0$ in the momentum-conserved stage) of bubbles 
%as a function of time when varying the initial conditions: temperature and 
%radius, as described in $\S$\ref{Sec:IniCon}, and as labelled.} 
%\label{ConvTest1a}
%\end{center}
%\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[width=0.47\textwidth]{Figs/BubblesTesting_InitialCond_1b_Bow06.BR.SNdyn.eps}
%\caption{Convergence test for the initial conditions of the SNe dynamical model. Panels are as in 
%Fig.~\ref{ConvTest1a}.} 
%\label{ConvTest1b}
%\end{center}
%\end{figure}
%\begin{figure}
%\begin{center}
%\includegraphics[width=0.47\textwidth]{Figs/BubblesTesting_InitialCond_1c_Bow06.BR.SNdyn.eps}
%\caption{Convergence test for the initial conditions of the SNe dynamical model. 
%Fig.~\ref{ConvTest1a}.}
%\label{ConvTest1c}
%\end{center}
%\end{figure}



